Horseshoe Prior Bayesian Quantile Regression

This paper extends the horseshoe prior of Carvalho et al. (2010) to Bayesian quantile regression (HS-BQR) and provides a fast sampling algorithm for computation in high dimensions. The performance of the proposed HS-BQR is evaluated on Monte Carlo simulations and a high dimensional Growth-at-Risk (GaR) forecasting application for the U.S. The Monte Carlo design considers several sparsity and error structures. Compared to alternative shrinkage priors, the proposed HS-BQR yields better (or at worst similar) performance in coefficient bias and forecast error. The HS-BQR is particularly potent in sparse designs and in estimating extreme quantiles. As expected, the simulations also highlight that identifying quantile specific location and scale effects for individual regressors in dense DGPs requires substantial data. In the GaR application, we forecast tail risks as well as complete forecast densities using the McCracken and Ng (2020) database. Quantile specific and density calibration score functions show that the HS-BQR provides the best performance, especially at short and medium run horizons. The ability to produce well calibrated density forecasts and accurate downside risk measures in large data contexts makes the HS-BQR a promising tool for nowcasting applications and recession modelling.

==> backup.tex <==

\begin{table}[]
\centering
\begin{tabular}{r|c|ccccc}
\hline
 & KS & \multicolumn{5}{c}{Pseudo-$R^2$} \\
 $p$ &  & 0.05 & 0.25 & 0.5 & 0.75 & 0.95 \\
 \hline
 \hline
HS-BQR & 0.217 & 0.247 & 0.142 & 0.204
 & 0.176 & 0.18 \\
LBQR &  0.364** & 0.056 & 0.017 & 0.046 & 0.023 & 0.015 \\
BQRENET & 0.426*** & 0.054 & 0.052 & 0.12 & 0.026 & 0.01 \\
BALQR & 0.433*** & 0.001 & 0 & 0.033 & 0.019 & 0.078 \\
\hline
\end{tabular}
\caption{Performance of the different estimators for 2-step-ahead quantile forecasts. The first column, KS, reports the Kolmogorov-Smirnov test for equality to a uniform CDF with critical values of 0.374. 0.312 and 0.28 for the 1\%, 5\% and 10\% critical values respectively (indicated by ***,** and *). Pseudo-$R^2$ are shown the right most panel for a set of 5 chosen quantile levels.}
\label{tab:fitofestimates}
\end{table}

\begin{table}[]
\centering
\begin{tabular}{r|c|ccccc}
\hline
 & KS & \multicolumn{5}{c}{Pseudo-$R^2$} \\
 $p$ &  & 0.05 & 0.25 & 0.5 & 0.75 & 0.95 \\
 \hline
 \hline
HS-BQR & 0.247 & 0.158 & 0.117 & 0.147
 & 0.101 & 0.188 \\
LBQR &  0.333** & 0.003 & 0.006 & 0.019 & 0.024 & 0.064 \\
BQRENET & 0.402*** & 0.043 & 0.058 & 0.103 & 0.067 & 0.011 \\
BALQR & 0.491*** & 0.007 & 0.002 & 0.008 & 0.058 & 0.076 \\
\hline
\end{tabular}
\caption{Performance of the different estimators for 3-step-ahead quantile forecasts. The first column, KS, reports the Kolmogorov-Smirnov test for equality to a uniform CDF with critical values of 0.374. 0.312 and 0.28 for the 1\%, 5\% and 10\% critical values respectively (indicated by ***,** and *). Pseudo-$R^2$ are shown the right most panel for a set of 5 chosen quantile levels.}
\label{tab:fitofestimates}
\end{table}

\begin{table}[]
\centering
\begin{tabular}{r|c|ccccc}
\hline
 & KS & \multicolumn{5}{c}{Pseudo-$R^2$} \\
 $p$ &  & 0.05 & 0.25 & 0.5 & 0.75 & 0.95 \\
 \hline
 \hline
HS-BQR & 0.193 & 0.296 & 0.13 & 0.132
 & 0.111 & 0.071 \\
LBQR &  0.398** & 0.015 & 0.014 & 0.051 & 0.008 & 0.01 \\
BQRENET & 0.370** & 0.023 & 0.01 & 0.063 & 0.008 & 0.001 \\
BALQR & 0.446*** & 0.052 & 0 & 0.017 & 0.035 & 0.088 \\
\hline
\end{tabular}
\caption{Performance of the different estimators for 4-step-ahead quantile forecasts. The first column, KS, reports the Kolmogorov-Smirnov test for equality to a uniform CDF with critical values of 0.374. 0.312 and 0.28 for the 1\%, 5\% and 10\% critical values respectively (indicated by ***,** and *). Pseudo-$R^2$ are shown the right most panel for a set of 5 chosen quantile levels.}
\label{tab:fitofestimates}
\end{table}

\begin{table}[]
\centering
\begin{tabular}{rccccc}
\hline
 \multicolumn{5}{c}{Average Log-Scores} \\
  & h=1 & h=2 & h=3 & h=4 \\
 \hline
 \hline
HS-BQR & 3.432 & 3.282 & 3.472
 & 3.534 \\
LBQR & 3.235 & 3.294 & 3.396 & 3.431 \\
BQRENET & 2.999 & 3.369 & 3.426 & 3.430 \\
BALQR & 1.839 & 2.069 & 2.154 & 2.133 \\
SPF & 3.083 & 3.276 & 3.285 & 3.185 \\
\hline
\end{tabular}
\caption{Average log scores of the different estimators for 1-,2-,3- and 4-step-ahead quantile forecasts. Density is approximated by a normal kernel of the 19 forecasted quantiles.}
\label{tab:logscores}
\end{table}

\begin{table}[]
\centering
\begin{tabular}{rccccc}
\hline
 \multicolumn{5}{c}{Median Quantile Forecasts} \\
  & h=1 & h=2 & h=3 & h=4 \\
 \hline
 \hline
HS-BQR & 0.006 & 0.004 & 0.004 & 0.004 \\
LBQR & 0.010*** & 0.012*** & 0.008*** & 0.008*** \\
BQRENET & 0.009*** & 0.007*** & 0.007*** & 0.008*** \\
BALQR & 0.015*** & 0.012*** & 0.010*** & 0.007*** \\
SPF & 0.005*** & 0.004*** & 0.004*** & 0.004*** \\
\hline
\end{tabular}
\caption{Mean-squared-forecast-errors based on the median quantiles for the different estimators for 1-,2-,3- and 4-step-ahead quantile forecasts. Stars indicate statistical difference to the HSBQR median forecasts based on the Diebold-Mariano test (1998) at 10\%, 5\% and 1\% significance respectively.}
\label{tab:MSFE}
\end{table}

% MANY ROWS 
\begin{table}[]
\centering
\begin{tabular}{rccccc}
\hline
  & h=1 & h=2 & h=3 & h=4 \\
 \hline
 \hline
 \multicolumn{5}{c}{Average Log-Scores} \\
 \hline
HS-BQR & 3.432 & 3.282 & 3.472
 & 3.534 \\
LBQR & 3.235 & 3.294 & 3.396 & 3.431 \\
BQRENET & 2.999 & 3.369 & 3.426 & 3.430 \\
BALQR & 1.839 & 2.069 & 2.154 & 2.133 \\
SPF & 3.083 & 3.276 & 3.285 & 3.185 \\
\hline
 \multicolumn{5}{c}{Median Quantile Forecasts} \\
 \hline
HS-BQR & 0.006 & 0.004 & 0.004 & 0.004 \\
LBQR & 0.010*** & 0.012*** & 0.008*** & 0.008*** \\
BQRENET & 0.009*** & 0.007*** & 0.007*** & 0.008*** \\
BALQR & 0.015*** & 0.012*** & 0.010*** & 0.007*** \\
SPF & 0.005*** & 0.004*** & 0.004*** & 0.004*** \\
\hline
\end{tabular}
\caption{Average log scores and the mean-squared-forecast errors of the median of the different estimators for 1-,2-,3- and 4-step-ahead quantile forecasts. Density for the log scores is approximated by a normal kernel of the 19 forecasted quantiles. Stars indicate statistical difference to the HSBQR median forecasts based on the Diebold-Mariano test (1998) at 10\%, 5\% and 1\% significance respectively.}
\label{tab:logscoresandMSFE}
\end{table}

%MANY COLUMNS
\begin{table}
\centering
\begin{tabular}{r|cccc|cccc}
\hline
 & \multicolumn{4}{c|}{Average Log-Scores} & \multicolumn{4}{c}{Median Quantile Forecasts}\\
  & h=1 & h=2 & h=3 & h=4 & h=1 & h=2 & h=3 & h=4 \\
 \hline
 \hline
HS-BQR & 3.432 & 3.282 & 3.472 & 3.534 & 0.006 & 0.004 & 0.004 & 0.004 \\
LBQR & 3.235 & 3.294 & 3.396 & 3.431 & 0.010*** & 0.012*** & 0.008*** & 0.008*** \\
BQRENET & 2.999 & 3.369 & 3.426 & 3.430 & 0.009*** & 0.007*** & 0.007*** & 0.008*** \\
BALQR & 1.839 & 2.069 & 2.154 & 2.133 & 0.015*** & 0.012*** & 0.010*** & 0.007*** \\
SPF & 3.083 & 3.276 & 3.285 & 3.185 & 0.005*** & 0.004*** & 0.004*** & 0.004***  \\
\hline
\end{tabular}
\caption{Average log scores and Mean-squared-forecast-errors on the median of the different estimators for 1-,2-,3- and 4-step-ahead quantile forecasts. Density is approximated by a normal kernel of the 19 forecasted quantiles. For the MSFE stars indicate statistical difference to the HSBQR median forecasts based on the Diebold-Mariano test (1998) at 10\%, 5\% and 1\% significance respectively.}
\label{tab:logscoresandMSFE}
\end{table}

%LONG TABLE
\begin{table}[]
\centering
\begin{tabular}{r|c|ccccc}
\hline
 & KS & \multicolumn{5}{c}{Pseudo-$R^2$} \\
  &  & 0.05 & 0.25 & 0.5 & 0.75 & 0.95 \\
 \hline
 \hline
 \multicolumn{7}{c}{\textit{1-step ahead}}\\
 \hline
HS-BQR & 0.195 & 0.256 & 0.13 & 0.102 & 0.15 & 0.234 \\
LBQR & 0.382*** & 0.049 & 0.083 & 0.028 & 0.031 & 0.067 \\
BQRENET & 0.396*** & 0.048 & 0.11 & 0.063 & 0.041 & 0.001 \\
BALQR & 0.443*** & 0.11 & 0.025 & 0 & 0.001 & 0.039 \\
 \hline
 \multicolumn{7}{c}{\textit{2-step ahead}}\\
 \hline
HS-BQR & 0.217 & 0.247 & 0.142 & 0.204 & 0.176 & 0.18 \\
LBQR &  0.364** & 0.056 & 0.017 & 0.046 & 0.023 & 0.015 \\
BQRENET & 0.426*** & 0.054 & 0.052 & 0.12 & 0.026 & 0.01 \\
BALQR & 0.433*** & 0.001 & 0 & 0.033 & 0.019 & 0.078 \\
 \hline
 \multicolumn{7}{c}{\textit{3-step ahead}}\\
 \hline
HS-BQR & 0.247 & 0.158 & 0.117 & 0.147 & 0.101 & 0.188 \\
LBQR &  0.333** & 0.003 & 0.006 & 0.019 & 0.024 & 0.064 \\
BQRENET & 0.402*** & 0.043 & 0.058 & 0.103 & 0.067 & 0.011 \\
BALQR & 0.491*** & 0.007 & 0.002 & 0.008 & 0.058 & 0.076 \\
 \hline
 \multicolumn{7}{c}{\textit{4-step ahead}}\\
 \hline
HS-BQR & 0.193 & 0.296 & 0.13 & 0.132 & 0.111 & 0.071 \\
LBQR &  0.398** & 0.015 & 0.014 & 0.051 & 0.008 & 0.01 \\
BQRENET & 0.370** & 0.023 & 0.01 & 0.063 & 0.008 & 0.001 \\
BALQR & 0.446*** & 0.052 & 0 & 0.017 & 0.035 & 0.088 \\
\hline
\end{tabular}
\caption{Performance of the different estimators for h-step-ahead quantile forecasts. The first column, KS, reports the Kolmogorov-Smirnov test for equality to a uniform CDF with critical values of 0.374. 0.312 and 0.28 for the 1\%, 5\% and 10\% critical values respectively (indicated by ***,** and *). Pseudo-$R^2$ are shown the right most panel for a set of 5 chosen quantiles}
\label{tab:fitofestimates}
\end{table}

%WIDE TABLE
\begin{table}[]
\centering
\resizebox{\textwidth}{!}{
\begin{tabular}{r|c|ccccc|c|ccccc}
\hline
 & KS & \multicolumn{5}{c|}{Pseudo-$R^2$}& KS & \multicolumn{5}{c}{Pseudo-$R^2$} \\
  &  & 0.05 & 0.25 & 0.5 & 0.75 & 0.95 &  & 0.05 & 0.25 & 0.5 & 0.75 & 0.95 \\
 \hline
 \hline
 & \multicolumn{6}{c|}{\textit{1-step ahead}} & \multicolumn{6}{c}{\textit{2-step ahead}}\\
 \hline
HS-BQR & 0.195 & 0.256 & 0.13 & 0.102 & 0.15 & 0.234 & 0.217 & 0.247 & 0.142 & 0.204 & 0.176 & 0.18 \\
LBQR & 0.382*** & 0.049 & 0.083 & 0.028 & 0.031 & 0.067 &  0.364** & 0.056 & 0.017 & 0.046 & 0.023 & 0.015 \\
BQRENET & 0.396*** & 0.048 & 0.11 & 0.063 & 0.041 & 0.001 & 0.426*** & 0.054 & 0.052 & 0.12 & 0.026 & 0.01 \\
BALQR & 0.443*** & 0.11 & 0.025 & 0 & 0.001 & 0.039 & 0.433*** & 0.001 & 0 & 0.033 & 0.019 & 0.078 \\
 \hline
 & \multicolumn{6}{c|}{\textit{3-step ahead}} & \multicolumn{6}{c}{\textit{4-step ahead}}\\
 \hline
HS-BQR & 0.247 & 0.158 & 0.117 & 0.147 & 0.101 & 0.188 & 0.193 & 0.296 & 0.13 & 0.132 & 0.111 & 0.071 \\
LBQR &  0.333** & 0.003 & 0.006 & 0.019 & 0.024 & 0.064 &  0.398** & 0.015 & 0.014 & 0.051 & 0.008 & 0.01 \\
BQRENET & 0.402*** & 0.043 & 0.058 & 0.103 & 0.067 & 0.011 & 0.370** & 0.023 & 0.01 & 0.063 & 0.008 & 0.001 \\
BALQR & 0.491*** & 0.007 & 0.002 & 0.008 & 0.058 & 0.076 & 0.446*** & 0.052 & 0 & 0.017 & 0.035 & 0.088 \\
 \hline
\end{tabular}}
\caption{Performance of the different estimators for h-step-ahead quantile forecasts. The first column, KS, reports the Kolmogorov-Smirnov test for equality to a uniform CDF with critical values of 0.374. 0.312 and 0.28 for the 1\%, 5\% and 10\% critical values respectively (indicated by ***,** and *). Pseudo-$R^2$ are shown the right most panel for a set of 5 chosen quantiles.}
\label{tab:fitofestimates}
\end{table}

\begin{comment}
% Please add the following required packages to your document preamble:
% \usepackage{graphicx}
% \usepackage{lscape}
\begin{landscape}
\begin{table}[]
\caption{Root mean coefficient bias for coefficients with non-constant quantile profile}
\label{tab:quantilebiasresults}
\centering
\resizebox{1.3\textwidth}{!}{%
\begin{tabular}{rrccccc|ccccc|ccccc|ccccc}
\hline
 & $p$ & 0.1 & 0.3 & 0.5 & 0.7 & 0.9 & 0.1 & 0.3 & 0.5 & 0.7 & 0.9 & 0.1 & 0.3 & 0.5 & 0.7 & 0.9 & 0.1 & 0.3 & 0.5 & 0.7 & 0.9 \\
 \hline
 \hline
 &  & \multicolumn{5}{c|}{$y_1$} & \multicolumn{5}{c|}{$y_2$} & \multicolumn{5}{c|}{$y_3$} & \multicolumn{5}{c}{$y_4$} \\
 \multicolumn{2}{l}{\textbf{T=100}} &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  \\
\multicolumn{2}{l}{Sparse} &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  \\
 & \textit{HS-BQR} & 0.515 & 0.295 & 0.104 & 0.348 & 0.757 & 0.723 & 0.315 & 0.137 & 0.380 & 1.014 & 0.521 & 0.535 & 0.815 & 1.187 & 1.752 & 0.470 & 0.448 & 0.725 & 1.087 & 1.644 \\
 %& \textit{L1-QR} & 0.070 & 0.056 & 0.051 & 0.056 & 0.069 & 0.093 & 0.078 & 0.076 & 0.079 & 0.095 & 0.133 & 0.143 & 0.149 & 0.147 & 0.142 & 0.096 & 0.089 & 0.088 & 0.093 & 0.103 \\
 & \textit{LBQR} & 0.418 & 0.165 & 0.399 & 0.891 & 1.572 & 0.692 & 0.253 & 0.522 & 0.949 & 1.884 & 12.375 & 3.206 & 4.505 & 3.076 & 4.246 & 13.274 & 2.569 & 4.337 & 3.557 & 4.405 \\
 & \textit{BQRENET} & 0.415 & 0.158 & 0.355 & 0.714 & 1.369 & 0.616 & 0.301 & 0.533 & 0.684 & 1.638 & 0.381 & 0.353 & 0.625 & 0.976 & 1.661 & 0.378 & 0.260 & 0.541 & 0.960 & 1.595 \\
 & \textit{BALQR} & 1.225 & 0.464 & 0.121 & 0.586 & 1.341 & 1.574 & 0.559 & 0.330 & 0.708 & 1.690 & 2.821 & 2.973 & 3.510 & 3.117 & 4.417 & 1.933 & 2.224 & 1.983 & 2.522 & 2.901 \\
\multicolumn{2}{l}{Dense} &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  \\
 & \textit{HS-BQR} & 0.480 & 0.451 & 0.769 & 1.164 & 1.654 & 0.816 & 0.427 & 0.778 & 1.218 & 1.990 & 1.037 & 0.612 & 0.708 & 1.012 & 1.573 & 0.645 & 0.953 & 1.297 & 1.657 & 1.962 \\
 %& \textit{L1-QR} & 0.897 & 0.890 & 0.889 & 0.891 & 0.910 & 0.902 & 0.900 & 0.899 & 0.899 & 0.917 & 0.918 & 0.923 & 0.925 & 0.922 & 0.940 & 0.912 & 0.908 & 0.907 & 0.908 & 0.928 \\
 & \textit{LBQR} & 0.483 & 0.473 & 0.704 & 0.980 & 1.154 & 0.635 & 0.457 & 0.703 & 0.873 & 1.408 & 0.951 & 0.630 & 0.740 & 0.973 & 1.396 & 0.744 & 0.608 & 0.652 & 0.998 & 1.341 \\
 & \textit{BQRENET} & 0.574 & 0.503 & 0.681 & 0.931 & 1.226 & 0.773 & 0.530 & 0.677 & 1.020 & 1.501 & 0.966 & 0.619 & 0.680 & 0.977 & 1.430 & 0.772 & 0.613 & 0.643 & 0.840 & 1.249 \\
 & \textit{BALQR} & 0.849 & 0.679 & 1.002 & 1.440 & 2.072 & 0.987 & 0.696 & 1.028 & 1.460 & 2.329 & 1.252 & 1.083 & 1.048 & 1.428 & 1.906 & 1.474 & 1.055 & 1.262 & 1.456 & 1.910 \\
\multicolumn{2}{l}{Block} &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  \\
 & \textit{HS-BQR} & 0.368 & 0.475 & 0.947 & 1.420 & 2.101 & 0.693 & 0.427 & 0.983 & 1.496 & 2.457 & 0.598 & 0.452 & 0.874 & 1.339 & 2.037 & 0.686 & 1.018 & 1.418 & 1.850 & 2.280 \\
 %& \textit{L1-QR} & 0.860 & 0.879 & 0.880 & 0.879 & 0.858 & 0.862 & 0.881 & 0.882 & 0.882 & 0.860 & 0.867 & 0.889 & 0.889 & 0.887 & 0.868 & 0.863 & 0.888 & 0.888 & 0.887 & 0.866 \\
 & \textit{LBQR} & 0.413 & 0.638 & 0.956 & 1.333 & 1.806 & 0.651 & 0.591 & 0.964 & 1.308 & 2.221 & 0.705 & 0.559 & 0.774 & 1.179 & 1.870 & 0.621 & 0.695 & 0.881 & 1.338 & 1.714 \\
 & \textit{BQRENET} & 0.509 & 0.551 & 0.958 & 1.317 & 1.814 & 0.644 & 0.594 & 0.905 & 1.255 & 2.082 & 0.393 & 0.408 & 0.752 & 1.199 & 1.751 & 0.677 & 0.662 & 0.882 & 1.240 & 1.761 \\
 & \textit{BALQR} & 0.458 & 0.457 & 0.927 & 1.450 & 2.115 & 0.754 & 0.407 & 0.928 & 1.487 & 2.497 & 1.302 & 0.869 & 0.605 & 1.122 & 1.730 & 0.728 & 0.907 & 1.315 & 1.756 & 2.323 \\
 \hline
 \multicolumn{2}{l}{\textbf{T=400}} &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  \\
 \multicolumn{2}{l}{Dense} &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  \\
 & \textit{HS-BQR} & 0.559 & 0.230 & 0.076 & 0.254 & 0.588 & 0.584 & 0.207 & 0.093 & 0.223 & 0.552 & 0.603 & 0.404 & 0.353 & 0.404 & 0.620 & 0.411 & 0.424 & 0.707 & 1.036 & 1.395 \\
 & \textit{LBQR} & 0.234 & 0.074 & 0.064 & 0.075 & 0.228 & 0.223 & 0.249 & 0.082 & 0.222 & 0.200 & 0.791 & 0.452 & 0.297 & 0.445 & 0.840 & 0.471 & 0.283 & 0.202 & 0.283 & 0.490 \\
 & \textit{BQRENET} & 0.236 & 0.071 & 0.062 & 0.065 & 0.230 & 0.208 & 0.240 & 0.081 & 0.207 & 0.194 & 0.748 & 0.430 & 0.279 & 0.378 & 0.728 & 0.458 & 0.271 & 0.183 & 0.260 & 0.467 \\
 & \textit{BALQR} & 0.216 & 0.077 & 0.064 & 0.070 & 0.193 & 0.248 & 0.269 & 0.083 & 0.237 & 0.240 & 0.918 & 0.463 & 0.327 & 0.502 & 1.018 & 0.466 & 0.297 & 0.201 & 0.272 & 0.475 \\
  \multicolumn{2}{l}{Block} &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  \\
 & \textit{HS-BQR} & 0.471 & 0.345 & 0.581 & 0.910 & 1.280 & 0.824 & 0.318 & 0.594 & 0.982 & 1.630 & 0.994 & 0.582 & 0.585 & 0.905 & 1.448 & 0.734 & 0.476 & 0.548 & 0.862 & 1.303 \\
 & \textit{LBQR} & 0.290 & 0.437 & 0.386 & 0.559 & 0.530 & 0.346 & 0.365 & 0.577 & 0.546 & 0.503 & 1.044 & 0.562 & 0.586 & 0.788 & 1.061 & 0.580 & 0.537 & 0.535 & 0.760 & 0.906 \\
 & \textit{BQRENET} & 0.364 & 0.353 & 0.403 & 0.573 & 0.526 & 0.434 & 0.299 & 0.560 & 0.569 & 0.890 & 0.941 & 0.662 & 0.481 & 0.752 & 0.993 & 0.596 & 0.528 & 0.578 & 0.731 & 0.971 \\
 & \textit{BALQR} & 0.770 & 0.530 & 0.733 & 1.043 & 1.493 & 1.497 & 0.536 & 0.754 & 1.200 & 2.207 & 1.302 & 0.869 & 0.605 & 1.122 & 1.730 & 0.954 & 0.621 & 0.836 & 1.098 & 1.577 \\
 \hline
\end{tabular}%
}
\end{table}
\end{landscape}
\end{comment}
